Supporting Developers in Addressing Human-centric Issues in Mobile Apps

Failure to consider the characteristics, limitations, and abilities of diverse end-users during mobile apps development may lead to problems for end-users such as accessibility and usability issues. We refer to this class of problems as human-centric issues. Despite their importance, there is a limited understanding of the types of human-centric issues that are encountered by end-users and taken into account by the developers of mobile apps. In this paper, we examine what human-centric issues end-users report through Google App Store reviews, which human-centric issues are a topic of discussion for developers on GitHub, and whether end-users and developers discuss the same human-centric issues. We then investigate whether an automated tool might help detect such human-centric issues and whether developers would find such a tool useful. To do this, we conducted an empirical study by extracting and manually analysing a random sample of 1,200 app reviews and 1,200 issue comments from 12 diverse projects that exist on both Google App Store and GitHub. Our analysis led to a taxonomy of human-centric issues that categorises human-centric issues into three-high levels: App Usage, Inclusiveness, and User Reaction. We then developed machine learning and deep learning models that are promising in automatically identifying and classifying human-centric issues from app reviews and developer discussions. A survey of mobile app developers shows that the automated detection of human-centric issues has practical applications. Guided by our findings, we highlight some implications and possible future work to further understand and incorporate human-centric issues in mobile apps development.

==> Figures/SurveyResponses.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{img/SurveyResponses.pdf}
\vspace{-3mm}
\caption{Participants' level of agreement with the statements}
\label{fig:survey}
\end{figure}

==> Tables/Results.tex <==
\begin{table*}[]
\centering
\caption{Number (\#) and percentage (\%) of human-centric issues in different projects}
\label{tbl:results}
{\scriptsize
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
                         & \multicolumn{2}{c|}{\textbf{Inclusiveness}} & \multicolumn{2}{c|}{\textbf{Privacy/security}} & \multicolumn{2}{c|}{\textbf{Compatibility}} & \multicolumn{2}{c|}{\textbf{Location/Language}} & \multicolumn{2}{c|}{\textbf{Preference}} & \multicolumn{2}{c|}{\textbf{Satisfaction}} & \multicolumn{2}{c|}{\textbf{Emotional aspects}} & \multicolumn{2}{c|}{\textbf{Accessibility}} \\ \hline
\textbf{Project}         & \textbf{\#}             & \textbf{\%}            & \textbf{\#}              & \textbf{\%}              & \textbf{\#}             & \textbf{\%}            & \textbf{\#}               & \textbf{\%}              & \textbf{\#}           & \textbf{\%}           & \textbf{\#}            & \textbf{\%}            & \textbf{\#}               & \textbf{\%}              & \textbf{\#}             & \textbf{\%}            \\ \hline
\textbf{Firefox-ios}     & 3                       & 0.82                   & 6                        & 1.63                     & 5                       & 1.36                   & 1                         & 0.27                     & 14                    & 3.81                  & 10                     & 2.72                   & 3                         & 0.82                     & 5                       & 1.36                   \\ \hline
\textbf{Cwa-app-ios}     & 14                      & 4.33                   & 11                       & 3.41                     & 13                      & 4.02                   & 18                        & 5.57                     & 5                     & 1.55                  & 17                     & 5.26                   & 3                         & 0.93                     & 4                       & 1.24                   \\ \hline
\textbf{Cwa-app-android} & 3                       & 1.66                   & 21                       & 11.60                    & 10                      & 5.52                   & 19                        & 10.50                    & 6                     & 3.31                  & 11                     & 6.08                   & 1                         & 0.55                     & 1                       & 0.55                   \\ \hline
\textbf{Healthchecks}    & 1                       & 0.34                   & 5                        & 1.71                     & 0                       & 0.00                   & 5                         & 1.71                     & 11                    & 3.75                  & 8                      & 2.73                   & 2                         & 0.68                     & 2                       & 0.68                   \\ \hline
%\textbf{Pedometer}       & 0                       & 0.00                   & 1                        & 0.63                     & 1                       & 0.63                   & 5                         & 3.13                     & 2                     & 1.25                  & 6                      & 3.75                   & 1                         & 0.63                     & 1                       & 0.63                   \\ \hline
\textbf{Mobile-ios}      & 2                       & 5.88                   & 4                        & 11.76                    & 4                       & 11.76                  & 1                         & 2.94                     & 6                     & 17.65                 & 5                      & 14.71                  & 0                         & 0.00                     & 0                       & 0.00                   \\ \hline
\textbf{Mobile-android}  & 0                       & 0.00                   & 15                       & 32.61                    & 1                       & 2.17                   & 0                         & 0.00                     & 4                     & 8.70                  & 6                      & 13.04                  & 1                         & 2.17                     & 0                       & 0.00                   \\ \hline
\textbf{Total}           & 23                      & 1.64                   & 63                       & 4.49                     & 34                      & 2.42                   & 49                        & 3.49                     & 48                    & 3.42                  & 63                     & 4.49                   & 11                        & 0.78                     & 13                      & 0.93                   \\ \hline
\end{tabular}
}
\end{table*}
